Answer Set Planning: A Survey

Answer Set Planning refers to the use of Answer Set Programming (ASP) to compute plans, i.e., solutions to planning problems, that transform a given state of the world to another state. The development of efficient and scalable answer set solvers has provided a significant boost to the development of ASP-based planning systems. This paper surveys the progress made during the last two and a half decades in the area of answer set planning, from its foundations to its use in challenging planning domains. The survey explores the advantages and disadvantages of answer set planning. It also discusses typical applications of answer set planning and presents a set of challenges for future research.

==> include/asp-macros/dtel.tex <==
\RequirePackage{bm}
\RequirePackage{textcomp}
\RequirePackage{upgreek}

\IfFileExists{outline.tex}{\input{outline}}{}

\newcommand{\tuple}[1]{\langle #1 \rangle}
\renewcommand{\H}{\ensuremath{\mathbf{H}}} % REDEFINITION
\newcommand{\T}{\ensuremath{\mathbf{T}}}
\newcommand{\M}{\ensuremath{\mathbf{M}}}

\newcommand{\next}{\text{\rm \raisebox{-.5pt}{\Large\textopenbullet}}}  % {{\ensuremath{\circ}}}
\newcommand{\previous}{\text{\rm \raisebox{-.5pt}{\Large\textbullet}}}  % {{\ensuremath{\bullet}}}
\newcommand{\wnext}{\ensuremath{\widehat{\next}}}
\newcommand{\wprevious}{\ensuremath{\widehat{\previous}}}
\newcommand{\alwaysF}{\ensuremath{\square}}
\newcommand{\alwaysP}{\ensuremath{\blacksquare}}
\newcommand{\eventuallyF}{\ensuremath{\Diamond}}
\newcommand{\eventuallyP}{\ensuremath{\blacklozenge}}
\IfFileExists{outline.tex}
        {\newcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}}
        {\newcommand{\until}{\ensuremath{\mathbin{\bm{\mathsf{U}}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}}
        {\newcommand{\release}{\ensuremath{\mathbin{\bm{\mathsf{R}}}}}}
\newcommand{\since}{\ensuremath{\mathbin{\bm{\mathsf{S}}}}}
\newcommand{\trigger}{\ensuremath{\mathbin{\bm{\mathsf{T}}}}}
\IfFileExists{outline.tex}
        {\newcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}}
        {\newcommand{\finally}{\ensuremath{\bm{\mathsf{F}}}}}
\newcommand{\initially}{\ensuremath{\bm{\mathsf{I}}}}

\newcommand{\stp}{\ensuremath{\uptau}}

\newcommand{\dalways}[1]{\ensuremath{[#1]\,}}                        % \DBox
\newcommand{\deventually}[1]{\ensuremath{\langle#1\rangle\,}}        % \DDia
\newcommand{\drel}[2]{\ensuremath{{\parallel}{#1}{\parallel}^{#2}}}  % \Rel

\newcommand{\intervc}[2]{[#1..#2]}
\newcommand{\intervo}[2]{[#1..#2)}
\newcommand{\ointerv}[2]{(#1..#2]}
\newcommand{\rangec}[3]{#1 \in \intervc{#2}{#3}}
\newcommand{\rangeo}[3]{#1 \in \intervo{#2}{#3}}
\newcommand{\orange}[3]{#1 \in \ointerv{#2}{#3}}


==> include/asp-macros/listings.tex <==
% The language definitions below require the following packages:
%
%     \usepackage{courier}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%     \renewcommand{\Underscore}{\textscale{1}{\textunderscore}}
%
% Without extra packages I had to provide an alternative underscore definition
% to get decent looking underscores.
%
% As an alternative to courier, it is also possible to use the `lmodern`
% package.
%
%     \usepackage[T1]{fontenc}
%     \usepackage{lmodern}
%     \usepackage{xcolor}
%     \usepackage{relsize}
%
%     \input{listings}
%
% When the python or clingo language is given, tex code can be embedded
% escaping it in `#( ... #)`, which is treated like a comment in Python.
% Furthermore, for logic programs the character sequence is `%%` is not output.
% This can be used to add labels at the end of lines. For example, in a logic
% program one can write
%
%     H :- B.%%#( \label{lst:rule} #)
%
% to refer to the rule from the document without having to worry about changing
% line numbers when refactoring. The annotated program will still be runnable
% with clingo.

\providecommand{\Underscore}{\textunderscore}

\lstdefinelanguage{clingo}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  keywordstyle=[2]\bfseries,%
  keywordstyle=[3]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}1 {\%\%}{}0,%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  keywords=[2]{\#const,\#show,\#minimize,\#base,\#theory,\#count,\#external,\#program,\#script,\#end,\#heuristic,\#edge,\#project,\#show,\#sum},%
  keywords=[3]{&,&dom,&sum,&diff,&show},%
  morecomment=[l]{\#\ },%
  morecomment=[l]{\%\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}

\lstdefinelanguage{python}{%
  basicstyle=\ttfamily,%
  keywordstyle=[1]\bfseries,%
  showstringspaces=false,%
  literate={_}{\Underscore}{1},%
  escapeinside={\#(}{\#)},%
  alsoletter={\#,\&},%
  keywords=[1]{not,from,import,def,if,else,elif,return,while,break,and,or,for,in,del,and,class,with,as,is,yield,async},%
  morecomment=[l]{\#\ },%
  morestring=[b]",%
  stringstyle={\itshape},%
  commentstyle={\color{darkgray}}%
}



==> include/asp-macros/logics.tex <==
\newcommand{\HT}{\ensuremath{\mathrm{HT}}}
\newcommand{\EL}{\ensuremath{\mathrm{EL}}}
%
\newcommand{\LTL}{\ensuremath{\mathrm{LTL}}}
\newcommand{\LTLf}{\ensuremath{\mathrm{LTL}_{\!f}}}
\newcommand{\LTLo}{\ensuremath{\mathrm{LTL}_{\omega}}}
\newcommand{\THT}{\ensuremath{\mathrm{THT}}}
\newcommand{\THTf}{\ensuremath{\mathrm{THT}_{\!f}}}
\newcommand{\THTo}{\ensuremath{\mathrm{THT}_{\!\omega}}}
\newcommand{\TEL}{\ensuremath{\mathrm{TEL}}}
\newcommand{\TELf}{\ensuremath{{\TEL}_{\!f}}}
\newcommand{\TELo}{\ensuremath{{\TEL}_{\omega}}}
%
\newcommand{\LDL}{\ensuremath{\mathrm{LDL}}}
\newcommand{\LDLf}{\ensuremath{\mathrm{LDL}_{\!f}}}
\newcommand{\LDLo}{\ensuremath{\mathrm{LDL}_{\omega}}}
\newcommand{\DHT}{\ensuremath{\mathrm{DHT}}}
\newcommand{\DHTf}{\ensuremath{\mathrm{DHT}_{\!f}}}
\newcommand{\DHTo}{\ensuremath{\mathrm{DHT}_{\!\omega}}}
\newcommand{\DEL}{\ensuremath{\mathrm{DEL}}}
\newcommand{\DELf}{\ensuremath{{\DEL}_{\!f}}}
\newcommand{\DELo}{\ensuremath{{\DEL}_{\omega}}}
%
\newcommand{\DL}{\ensuremath{\mathrm{DL}}}


==> include/asp-macros/nogoods.tex <==
\newcommand{\domain}[1]{\ensuremath{\mathit{dom}(#1)}}

\newcommand{\ass}{\ensuremath{A}}

\newcommand{\tlits}[1]{\ensuremath{{#1}^{\true}}}
\newcommand{\flits}[1]{\ensuremath{{#1}^{\false}}}
\newcommand{\prefix}[2]{\ensuremath{#1[#2]}}

% \newcommand{\clno}[1]{\ensuremath{\delta(#1)}}
% \newcommand{\ClNo}[1]{\ensuremath{\Delta(#1)}}
% \newcommand{\nocl}[1]{\ensuremath{\gamma(#1)}}
% \newcommand{\NoCl}[1]{\ensuremath{\Gamma(#1)}}

\newcommand{\CN}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\LN}[1]{\ensuremath{\Lambda_{#1}}}

\newcommand{\dl}[0]{\ensuremath{\mathit{dl}}}
\newcommand{\dlevel}[1]{\ensuremath{\mathit{dlevel}(#1)}}
\newcommand{\opp}[1]{\ensuremath{\overline{#1}}}

\newcommand{\undef}[0]{\ensuremath{\circ}}
\newcommand{\trdef}[0]{\ensuremath{\times}}
\newcommand{\scc}[1]{\ensuremath{\mathit{scc}(#1)}}
\newcommand{\source}[1]{\ensuremath{\mathit{source}(#1)}}


==> include/asp-macros/operators.tex <==

% - operators ------------------------------------------------------------------
\newcommand{\Cn}[1]{\ensuremath{\mathit{Cn}(#1)}}
\newcommand{\reduct}[2]{\ensuremath{#1^{#2}}}

\newcommand{\Top}[1]{\ensuremath{T_{#1}}}
\newcommand{\T}[2]{\Top{#1}#2}
\newcommand{\Topi}[2]{\Top{#2}^{#1}}
\newcommand{\Ti}[3]{\Topi{#1}{#2}#3}

\newcommand{\BF}[1]{\ensuremath{\mathit{BF}(#1)}}
\newcommand{\CF}[1]{\ensuremath{\mathit{CF}(#1)}}
\newcommand{\CFIF}[1]{\ensuremath{\overleftarrow{\mathit{CF}}(#1)}}
\newcommand{\CFFI}[1]{\ensuremath{\overrightarrow{\mathit{CF}}(#1)}}
\newcommand{\CFX}[1]{\ensuremath{\mathit{CF}^x(#1)}}

\newcommand{\loops}[1]{\ensuremath{\mathit{loop}(#1)}}\message{*** loop already defined ***}
\newcommand{\ES}[2]{\ensuremath{\mathit{ES}_{\!#2}(#1)}}
\newcommand{\EB}[2]{\ensuremath{\mathit{EB}_{\!#2}(#1)}}
\newcommand{\LFM}[2]{\ensuremath{\mathit{LF}_{\!#2}(#1)}}
\newcommand{\LF}[1]{\ensuremath{\mathit{LF}(#1)}}

% - semantic operators -----------------------------------------------------------
\newcommand{\SM}[1]{\ensuremath{\mathit{SM}(#1)}}


==> include/asp-macros/outline.tex <==
\RequirePackage{xcolor}
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> include/asp-macros/planners.tex <==

\def\naf{{ not \:}}
\def\iif{\hbox{\bf if } \; }
\def\tthen{\; \hbox{\bf then } \; }
\def\eelse{\; \hbox{\bf else } \; }
\def\causes{\hbox{\bf causes}}
\def\caused{\hbox{\bf caused}}
\def\executable{\hbox{\bf executable}}
\def\initially{\hbox{\bf initially}}
\def\lan{\langle}
\def\ran{\rangle}
\def\cpasp{{\sc CPasp}}
\def\determines{\hbox{\bf determines}}
\def\oneof{\hbox{\bf oneof}}
\def\kcases{{\bf cases}}
\def\cps{{\sc ASPcp}}
\def\sgp{SGP}
\def\ccalc{CCalc}
\def\cmbp{CMBP}
\def\cps{LCP}
\def\cpasp{{\sc CPasp}}
\def\pddl{PDDL}
\def\ar{{\mathcal{AR}}}
\def\opt{{\tt opt}}
\def\limit{{\tt limit}}
\def\kacmbp{KACMBP}
\def\cpa{{\sc CpA}}
\def\pond{POND}
\def\cff{CFF}
\def\cplan{$\cal C$-{\sc Plan}}
\def\lp{{lp}}
\def\cpaph{{\sc CPA$^{ph}$}}
\def\cpapc{{\sc CPA$^{pc}$}}
\def\cpa{{\textnormal{\sc CpA}}}
\def\fcpa{{\sc fCpA}}
\def\cf2cff{{\tt cf2cs(ff)}}

\def\cpls{{\tt CpLs}}

\def\t0{{\tt t0}}
\def\T1{{\tt t1}}

\def\tone{{\tt t1}}

\def\pond{{\sc POND}}
\def\ff{{\sc FF}}
\def\cff{{\sc CFF}}
\def\kacmbp{{\sc KACMBP}}
\def\dnf{{\sc DNF}}
\def\cnf{{\sc CNF}}
\def\pcnf{{\sc Prime-CNF}}
\def\cplan{{\sc C-Plan}}
\def\fragplan{{\sc Frag-Plan}}
\def\cplama{{\sc GC}$[\Omega]$}
\def\cplamas{{\sc GC}[LAMA]}
\def\gclama{{\sc GC}[LAMA]}
\def\ffreplan{{\sc FF}-Replan}

\def\Effect{{\mathit{Effect}}}
\def\dnf{{\sc Dnf}}
\def\cnf{{\sc Cnf}}
\def\pip{{\sc PIP}}


\def\until{\hbox{\bf until}}
\def\always{\hbox{\bf always}}
\def\eventually{\hbox{\bf eventually}}
\def\next{\hbox{\bf next}}
\def\goal{\hbox{\bf goal}}

%\renewcommand{\sysfont}{\textsc}
\newcommand{\dlvk}{\dlv$^\mathcal{K}$}




==> include/asp-macros/syntax.tex <==
\newcommand{\naf}[1]{\ensuremath{{\sim\!{#1}}}}

\newcommand{\head}[1]{\ensuremath{\mathit{head}(#1)}}
\newcommand{\body}[1]{\ensuremath{\mathit{body}(#1)}}

\newcommand{\atom}[1]{\ensuremath{\mathit{atom}(#1)}}

\newcommand{\poslits}[1]{\ensuremath{{#1}^+}}
\newcommand{\neglits}[1]{\ensuremath{{#1}^-}}

\newcommand{\pbody}[1]{\poslits{\body{#1}}}
\newcommand{\nbody}[1]{\neglits{\body{#1}}}

\newcommand{\PRG}{\ensuremath{P}}

\newcommand{\atbody}[2]{\ensuremath{\mathit{body}_{#1}(#2)}}

\newcommand{\ground}[1]{\ensuremath{\mathit{grd}(#1)}}


==> include/asp-macros/tableau.tex <==
\newcommand{\true}{\ensuremath{\boldsymbol{T}}}
\newcommand{\false}{\ensuremath{\boldsymbol{F}}}

\newcommand{\Tsigned}[1]{\ensuremath{\true{#1}}}\message{ *** RENAME, Tlit,Flit ?? *** }
\newcommand{\Fsigned}[1]{\ensuremath{\false{#1}}}

\newcommand{\TOP}[1]{\ensuremath{D_{#1}}}
\newcommand{\COP}[1]{\ensuremath{D^*_{#1}}}

\newcommand{\Proviso}[1]{\raisebox{-7pt}[0pt][0pt]{\ensuremath{(#1)}}}

\newcommand{\plit}[1]{\ensuremath{\boldsymbol{t}{#1}}}
\newcommand{\nlit}[1]{\ensuremath{\boldsymbol{f}{#1}}}


==> systems.tex <==
\newcommand{\sysfont}{\textit}

\newcommand{\Clingo}{\sysfont{Clingo}}
\newcommand{\acthex}{\sysfont{acthex}}
\newcommand{\adsolver}{\sysfont{adsolver}}
\newcommand{\anthem}{\sysfont{anthem}}
\newcommand{\asparagus}{\sysfont{asparagus}}
\newcommand{\aspartame}{\sysfont{aspartame}}
\newcommand{\aspcud}{\sysfont{aspcud}}
\newcommand{\aspic}{\sysfont{aspic}}
\newcommand{\aspmt}{\sysfont{aspmt}}
\newcommand{\asprilo}{\sysfont{asprilo}}
\newcommand{\asprin}{\sysfont{asprin}}
\newcommand{\assat}{\sysfont{assat}}
\newcommand{\autofolio}{\sysfont{autofolio}}
\newcommand{\berkmin}{\sysfont{berkmin}}
\newcommand{\caspo}{\sysfont{caspo}}
\newcommand{\chasp}{\sysfont{chasp}}
\newcommand{\chuffed}{\sysfont{chuffed}}
\newcommand{\claspD}{\sysfont{claspD}}
\newcommand{\claspar}{\sysfont{claspar}}
\newcommand{\claspfolio}{\sysfont{claspfolio}}
\newcommand{\claspre}{\sysfont{claspre}}
\newcommand{\clasp}{\sysfont{clasp}}
\newcommand{\clingcon}{\sysfont{clingcon}}
\newcommand{\clingo}{\sysfont{clingo}}
\newcommand{\cmodels}{\sysfont{cmodels}}
\newcommand{\coala}{\sysfont{coala}}
\newcommand{\cplex}{\sysfont{cplex}}
\newcommand{\dflat}{\sysfont{dflat}}
\newcommand{\dingo}{\sysfont{dingo}}
\newcommand{\dlvhex}{\sysfont{dlvhex}}
\newcommand{\dlv}{\sysfont{dlv}}
\newcommand{\eclingo}{\sysfont{eclingo}}
\newcommand{\embasp}{\sysfont{embasp}}
\newcommand{\ezcsp}{\sysfont{ezcsp}}
\newcommand{\ezsmt}{\sysfont{ezsmt}}
\newcommand{\fastdownward}{\sysfont{fastdownward}}
\newcommand{\ftolp}{\sysfont{f2lp}}
\newcommand{\gasp}{\sysfont{gasp}}
\newcommand{\gecode}{\sysfont{gecode}}
\newcommand{\gfd}{\sysfont{g12fd}}
\newcommand{\gidl}{\sysfont{gidl}}
\newcommand{\ginkgo}{\sysfont{ginkgo}}
\newcommand{\gnt}{\sysfont{gnt}}
\newcommand{\gringo}{\sysfont{gringo}}
\newcommand{\harvey}{\sysfont{harvey}}
\newcommand{\iclingo}{\sysfont{iclingo}}
\newcommand{\idlv}{\sysfont{idlv}}
\newcommand{\idp}{\sysfont{idp}}
\newcommand{\inca}{\sysfont{inca}}
\newcommand{\jdlv}{\sysfont{jdlv}}
\newcommand{\lctocasp}{\sysfont{lc2casp}}
\newcommand{\lparse}{\sysfont{lparse}}
\newcommand{\lpsolve}{\sysfont{lpsolve}}
\newcommand{\lptodiff}{\sysfont{lp2diff}}
\newcommand{\lptosat}{\sysfont{lp2sat}}
\newcommand{\mchaff}{\sysfont{mchaff}}
\newcommand{\measp}{\sysfont{measp}}
\newcommand{\metasp}{\sysfont{metasp}}
\newcommand{\mingo}{\sysfont{mingo}}
\newcommand{\minisatid}{\sysfont{minisatid}}
\newcommand{\minisat}{\sysfont{minisat}}
\newcommand{\minizinc}{\sysfont{minizinc}}
\newcommand{\mznfzn}{\sysfont{mzn2fzn}}
\newcommand{\nomorepp}{\sysfont{nomore++}}
\newcommand{\oclingo}{\sysfont{oclingo}}
\newcommand{\omiga}{\sysfont{omiga}}
\newcommand{\picatsat}{\sysfont{picatsat}}
\newcommand{\picat}{\sysfont{picat}}
\newcommand{\piclasp}{\sysfont{piclasp}}
\newcommand{\picosat}{\sysfont{picosat}}
\newcommand{\plasp}{\sysfont{plasp}}
\newcommand{\qasp}{\sysfont{qasp}}
\newcommand{\quontroller}{\sysfont{quontroller}}
\newcommand{\reify}{\sysfont{reify}}
\newcommand{\rosoclingo}{\sysfont{rosoclingo}}
\newcommand{\sag}{\sysfont{sag}}
\newcommand{\satz}{\sysfont{satz}}
\newcommand{\siege}{\sysfont{siege}}
\newcommand{\smac}{\sysfont{smac}}
\newcommand{\smodelscc}{\sysfont{smodels$_{\!cc}$}}
\newcommand{\smodelsr}{\sysfont{smodels}$_r$}
\newcommand{\smodels}{\sysfont{smodels}}
\newcommand{\stelp}{\sysfont{stelp}}
\newcommand{\sugar}{\sysfont{sugar}}
\newcommand{\teaspoon}{\sysfont{teaspoon}}
\newcommand{\tefoli}{\sysfont{tefoli}}
\newcommand{\telingo}{\sysfont{telingo}}
\newcommand{\tel}{\sysfont{tel}}
\newcommand{\unclasp}{\sysfont{unclasp}}
\newcommand{\wasp}{\sysfont{wasp}}
\newcommand{\xorro}{\sysfont{xorro}}
\newcommand{\zchaff}{\sysfont{zchaff}}
\newcommand{\zzz}{\sysfont{z3}}

\newcommand{\clingoM}[1]{\clingo{\small\textnormal{[}\textsc{#1}\textnormal{]}}}
\newcommand{\ASPm}[1]{ASP\raisebox{.7pt}{[\textsc{#1}]}}

\newcommand{\flatzinc}{\sysfont{FlatZinc}}
\newcommand{\aspif}{\sysfont{aspif}}

\newcommand{\C}{C}
\newcommand{\cpp}{C++}
\newcommand{\haskell}{Haskell}
\newcommand{\java}{Java}
\newcommand{\lua}{Lua}
\newcommand{\prolog}{Prolog}
\newcommand{\python}{Python}
\newcommand{\rust}{Rust}

